Robustness May Be at Odds with Accuracy

We show that there may exist an inherent tension between the goal of adversarial robustness and that of standard generalization. Specifically, training robust models may not only be more resource-consuming, but also lead to a reduction of standard accuracy. We demonstrate that this trade-off between the standard accuracy of a model and its robustness to adversarial perturbations provably exists in a fairly simple and natural setting. These findings also corroborate a similar phenomenon observed empirically in more complex settings. Further, we argue that this phenomenon is a consequence of robust classifiers learning fundamentally different feature representations than standard classifiers. These differences, in particular, seem to result in unexpected benefits: the representations learned by robust models tend to align better with salient data characteristics and human perception.

==> linear_stuff.tex <==
We train a binary linear classifier to discriminate between ``5'' and ``7'' digits in the MNIST~\citep{mnist} dataset. In our training we learn the parameters $w \in \mathbb{R}^{784}$ and $b \in \mathbb{R}$, and minimize the cross-entropy loss with logits defined by the affine transform of the input data:
\begin{equation}
  \label{eq:binary-linear}
  \langle\cdot,w\rangle + b
\end{equation}
We set ``5'' to be in the ``negative'' direction and ``7'' to be in the ``positive'' direction of the linear classifier. \logan{there's definitely a better way of saying this} In each training routine we use, we perform $100$ epochs worth of gradient descent over the MNIST training set. We use two variants of training:

\begin{enumerate}
\item \textbf{Standard training: } In each training step we directly train on the unmodified images from the training set.
\item \textbf{Adversarial training: } In each training step we first adversarially perturb each image to optimally maximize the loss, then perform our training step on these adversarially perturbed images. The adversary here operates in the $\ell_\infty$ threat model, and has a budget of $\epsilon_{\infty} = 0.2$. The optimal step, as shown in \logan{was this shown earlier?? prob}, corresponds to adding $\pm\epsilon$ to each coordinate as to maximimally shift the affine function seen in Equation~(\ref{eq:binary-linear}) in the adversarial direction.\logan{prob should just make this explicit instead of explaining it}
\end{enumerate}

We evaluate each classifer we train on its standard test accuracy and on its adversarial test accuracy, which is the accuracy achieved when an adversary can perturb the input image with a $\epsilon_\infty = 0.20$ budget in the $\ell_\infty$ threat model.



